Fundamental Notions of Projective and Scale-Translation-Invariant Metrics in Coding Theory

Projective metrics on vector spaces over finite fields, introduced by Gabidulin and Simonis in 1997, generalize classical metrics in coding theory like the Hamming metric, rank metric, and combinatorial metrics. While these specific metrics have been thoroughly investigated, the overarching theory of projective metrics has remained underdeveloped since their introduction. In this paper, we present and develop the foundational theory of projective metrics, establishing several elementary key results on their characterizing properties, equivalence classes, isometries, constructions, connections with the Hamming metric, associated matroids, sphere sizes and Singleton-like bounds. Furthermore, some general aspects of scale-translation-invariant metrics are examined, with particular focus on their embeddings into larger projective metric spaces.

==> Sections/0-ideas.tex <==

\section*{Ideas}
\label{sec:ideas}
\addcontentsline{toc}{section}{\nameref{sec:ideas}}

Legend: \textcolor{green}{Question answered }, \textcolor{blue}{question answered but leading to other questions} \textcolor{violet}{Question to be answered, important and difficult}, \textcolor{gray}{not yet explored question}, explored question but without any useful result yet
\begin{itemize}
    \item \textcolor{green}{Counterimage of perfect code is also perfect?}
    \item operations on $\cF$ which give equivalent projective metrics (linear combination of rows ecc)
    \item \textcolor{green}{generalise definition of projective metrics to non spanning families}.
    \item \textcolor{blue}{Relation to matroids: are sphere sizes invariant by matroid isomorphism?} short answer: no. But other matroids could be considered. What is the smallewst matroid for which is true?
    \item more on new weights constructions: adding one vector to a spanning family
    \item Checking details about the ``more useful" Singleton bound.
    \item \textcolor{violet}{Can we generalize other bounds?}
    \item Checking details about the tensor-product construction.
    \item \textcolor{green}{Look that with the size of the spheres of the phase metric and by using "splitting" we have a formula for the size of spheres for all the projective metrics with size $\N = N + 1$.}
    \item \textcolor{green}{For ever $f\in \cF$ we can consider the "removal weight" of f: $w_{\cF\setminus \{f\}}(f)$. I think that a linear equivalence $L$ from $\cF$ to $\cF'$ for all $f \in \cF$ preserves the removal weight. Thus two equivalent projective metrics have the same removal weight distribution. I was wondering weather the opposite is true, that is weather two projective metric with the same removal weight distribution are always equivalent.} answer: no.
    \item \textcolor{violet}{Implementing in Sage, might be difficult since calculating weights is in general hard.} Implemented a slow algorithm, other shortest path ideas could be explere, implementation could use some polishing.
    \item \textcolor{gray}{Looking at other operations on the families, see how the corresponding parent codes look like (there should be much literature on combining codes).}
    \item \textcolor{gray}{Studying which properties from a parent-code, e.g. coset-leader weight distribution, transfer to properties of the corresponding projective metrics, e.g the size of the spheres. Can we get an asymptotic bound on the spheres, like you did for cover metric?}
    \item Transforming nice codes in Hamming metric containing the parent code   to   nice codes for projective metrics.
    \item General ISD for projective metrics? For example, a support of vector x could be a minimal subset of F containing x in its span?
    \item \textcolor{violet}{For codes attaining the singleton bounds (MFD? codes), is their dual code also MFD?} With the Hamming definition of dual codes no, we also explored some other possible definition but we also found counter examples to those. \emph{What could be a useful definition of duality?}
\end{itemize}


\hsc[inline]{As Anna noticed, it is computationally hard (NP-hard) to calculate the $\F$-weight of a vector for general $\F$. For example, for tensor codes it is mentioned in \cite{roth1996tensor}:  \textit{``\ldots unlike the matrix case, deciding upon the value of the rank of a tensor is known to be NP-hard''}.\\ 
- Nevertheless, for a particular metric, like Hamming or (matrix) Rank, it might be easy to calculate the weight.\\
- New metrics in which calculating the weight might be easy:  Phase-Rotating/Repetition code: \cite{gabidulin1998hard}, Vandermonde/GRS code: \cite{gabidulin2003codes}, \cite{catterall2006public}, Binary BCH code: \cite{gabidulin1998perfect}.
}
\gr[inline]{- If a decoding algorithm for $\C$ is known this is equivalent to knowing an algorithm for calculating the $\cF$-weight (as seen in Proposition (yet to add).}


\subsection*{Papers}


\begin{itemize}
    \item Recommended to start with, contains some details and proofs: \cite{gabidulin2003codes}.
    
    \item Coset leaders (also known to be very hard to compute the weight enumerator of): \cite{helleseth1979weight}, \cite{jurrius2009extended}.

    \item The three original short papers by Gabidulin and Simonis: \cite{gabidulin1997metrics}, \cite{gabidulin1998metrics}, \cite{gabidulin1998perfect}.

    \item Application to cryptography, but only with the ``Vandermonde $\F$-metric'': \cite{gabidulin2003codes}, \cite{catterall2006public}.

    \item Two general surveys: \cite{firer2021alternative}, \cite{gabidulin2012brief}.

    \item On the phase rotation metric, shows how to obtain good codes for this metric: \cite{gabidulin1998hard}.

    \item Tensor codes: \cite{roth1996tensor}, \cite{byrne2019tensor}, \cite{byrne2021tensor}.
\end{itemize}


\newpage
\textbf{Contents:}
\begin{enumerate}
\setcounter{enumi}{-1}
\item Notation
\item Intro/motivation/known examples (non-mathematical)
\item General definition (like gabidulin,simonis), reduce to projective weights with spanning families of 1-d subspaces.
\item Basic properties (triangle ineq, etc)
\item definition of parent codes (gabidulin,simonis),  (mention F weight corresponds to Hamming weight cosets,  prop: if hamming weight less (d-1)/2, then F-weight same) 
\item Examples (mathematical)



\item \textbf{Codes}\\
General code construction ideas (if exists a code in hamming metric containing parent code, then applying parent function gives code for F-metric)\\ (Equivalence codes in F-metric and Hamming codes containing parent code,   dual of parent is not parent of dual?)
\item Singleton bound
\item Spheres packing /hamming bound?
\item Perfect codes



\item \textbf{Details about metric spaces}\\ Calculating the weight (recursive algorithm) (decoding algorithm for parent codes)

\item Equivalence of projective metrics (including parent codes, and matroids?)
\item F-isometries
\item Constructing metrics with operations (including parent codes)

\end{enumerate}

\text{}\\
\textcolor{gray}{gray: no one checked}\\
\textcolor{violet}{violet: gabor checked, hugo not yet}\\
\textcolor{blue}{blue: hugo checked, gabor not yet}\\
black: both checked (at least once)
\newpage

Structure of introduction: (very little math)\\
\begin{itemize}
    \item History of the theory (first few papers, several later papers finding applications)
    \item % this can be first item
    Motivation/applications/importance/connections to other fields
    \item Summary of what has been done already, and what could be done in future (current state of research)
    \item Our contribution
    \item Structure of the paper (outline)
\end{itemize}

Summary/survey of existing literature:
\begin{itemize}
    \item \cite{gabidulin1997metrics} Gabidulin Simonis 1997: 
    \begin{itemize}
        \item Projective metric definitions, spanning family 
        \item Examples: phase rotation metric, rank metric, 
        \item Connection to Hamming metric: parent code, projective weight is Hamming weight of coset, max weight is covering radius of parent code, coset weight distribution is projective weight distribution
        \item If parent code chosen on GV bound, we know approximate the coset distribution up to min distance, asymptotics
    \end{itemize}
    \item \cite{gabidulin1998metrics} Gabidulin Simonis 1998: 
    \begin{itemize}
        \item Same as 1997 paper, more elaborate
        \item Their prop 2: $d_H(\phi^{-1}(D)) = \min(d_\cF(D), d_H(\wp))$, or $d_H(\phi^{-1}(D)\setminus \wp) = d_\cF(D)$?
        \item Corollary 1: optimal linear codes come from optimal linear codes containing $\wp$.
        \item Use perfect codes as parent codes: know coset distribution
        \item Lemma 1: proof coset distribution of GV-bound codes
    \end{itemize}
    \item \cite{gabidulin1998hard} Gabidulin Bossert 1998:
    \begin{itemize}
        \item Phase rotation metric definition
        \item Sphere sizes, perfect codes for Phase rotarion metrics over \(\bF_2\)
    \end{itemize}
\end{itemize}


%add good explenation on motivation for projective metrics

==> Sections/2-Rest.tex <==




{\color{gray}




\section{Constructing metrics}
{
\color{violet}
\subsection{Adding a vector to a spanning family.}
A natural way to construct a new a projective weight is by adding a vector \(f \notin \cF\) to the spanning family \(\cF\) of a known metric. We have the following basic relation with the new projective weight.
\begin{observation}
Let \(\cF\) be a spanning family of \(V\) and \(f \in V\), then
    \[wt_{\cF\cup\{f\}}(x) = \min \{wt_{\cF}(x), \min_{a \in \bF\withoutzero}(wt_{\cF}(x-af)+1)\}\]
\end{observation}
\textcolor{gray}{This may give an other algorithm to calculate the weight recursevely.}
 
\begin{observation}
    The following relation holds between the balls of \(\cF\) and \(\cF \cup \{f\}\):
    \begin{equation}
        B_t^{\cF \cup \{f\}} = S_t^{\cF} \cup (B_{t-1}^{\cF} +  \langle f \rangle).
    \end{equation}
   \hspace{2cm} In particular for the inclusion-exclusion principle we have:
    \begin{equation}
    \label{eq: Balls sizes of F cup f}
        |B_t^{\cF \cup \{f\}}| = |S_t^{\cF}| + |B_{t-1}^{\cF}+ \langle f \rangle| - |S_t^{\cF} \cap (B_{t-1}^{\cF} \cap \langle f \rangle)|.
    \end{equation}
\end{observation}

Equation \eqref{eq: Balls sizes of F cup f} gives the following upper bound of the ball sizes of \(\cF \cup \{f\}\):
\begin{observation}
\begin{equation}
    |B_t^{\cF \cup \{f\}}| \leq |S_t^{\F}| + q|B_{t-1}^{\cF}|.
\end{equation}
Where \(q = |\bF|\).
\end{observation}
\begin{proof}
    The function \(F \) mapping \((v,p) \in B_{t-1}^{\cF} \times \bF\) to \(v+pf \in B_{t-1}^{\cF} +  \langle f \rangle\) is surjective, thus \(|B_{t-1}^{\cF} +  \langle f \rangle| \leq |B_{t-1}^{\cF}|q\). From this follows the observation.
\end{proof}

This bound is actually tight for any ball of radious \(t \leq \frac{wt_{\cF}(f)}{2}\).

\begin{proposition}
    For all \( t \leq \frac{wt_{\cF}(f)}{2}\) we have
    \begin{equation}
        |B_t^{\cF \cup \{f\}}| = |S_t^{\F}| + q|B_{t-1}^{\cF}|.
    \end{equation}
\end{proposition}
\begin{proof}
    We show that the function \(F\) introduced earlier is also injective for all \(t \leq \frac{wt_{\cF}(f)}{2}\). If \(F(v_1,p_1)= v_1 + p_1f = v_2 + p_2f = F(v_2,p_2)\) then \((p_2-p_1)f = v_1 - v_2 \in B_{2(t-1)}^{\cF}\), since \(wt_{\cF}(v_1-v_2) \leq wt_{\cF}(v_1) + wt_{\cF}(v_2) \leq 2(t_1)\). Thus if \(p_1 \neq p_2\), then \(f \in B_{2(t-1)}^{\cF}\) but \(wt_{\cF}(f) \geq 2t > 2(t-1)\). Thus \(p_1 = p_2\) and \(v_1 = v_2\). This shows that \(F\) is a bijectiond and \(|B_{t_1}^{\cF}| = q|B_{t-1}^{\cF}|\).
    To conclude we show that \(S_t^{\cF} \cap (B_{t-1}^{\cF}+\langle f \rangle) = \emptyset\). If exists \(v \in S_t^{\cF} \cap (B_{t-1}^{\cF}+\langle f \rangle) \). Then \( v = w + pf\) for some \(w \in B_{t-1}^{\cF}\) and \(p \neq 0\). Thus, \(pf = v-w\) and we have:
    \begin{equation}
        2t-1 < wt_{\cF}(f) = wt_{\cF}(v-w) \leq wt_{\cF}(v) + wt_{\cF}(w) \leq t + t- 1 = 2t -1 
    \end{equation}
    Which gives a contradiction, thus  \(S_t^{\cF} \cap (B_{t-1}^{\cF}+\langle f \rangle) = \emptyset\) and this concludes.
\end{proof}
}

\section{Codes}

}
\section{Yet to be sorted stuff:}

\subsection{Other matroid tries}


{
\color{gray}

% \textcolor{red}{not sure if true:}
% \begin{proposition}
%     Let \(F_1,\ldots,F_k \in M(\cF)\) such that \(\dim(\bigcap_{i =1}^k\langle F_i \rangle) = d\) then there exists a bases of circuits \(c_1,\ldots, c_d \subset \bigcup_{i=1}^k F_i\) that is 
%     \[
%     \langle v_{c_1},\ldots v_{c_d} \rangle = \bigcap_{i=1}^k \langle F_i\rangle.
%     \]
%     Such that for all \(i = 1,\ldots,d\) we have \(c_i \setminus \cup_{j \neq i}c_j \neq \emptyset\) and for all \(k\) we have \(c_i \cap F_k \neq \emptyset\).
% \end{proposition}

This last proposition does not have a generalization for intersections of more than two elements, it that where the case we would have that the sphere size would be invariant by equivalent as matroids, but this is not the case. 
\begin{example}
\gr[]{A counterexample I think here would be quite important to add this section.}
    There are Matroid equivalent projective metrics which do not have same sphere sizes
\end{example}

What we can do is to "complete" the matroid with other vectors so it has enough information do describe all the intersections.
\begin{theorem}
    If \(M(\cF) \equiv M(\cG)\) then \(|B^{\cF}_t|=|B^{\cG}_t|\) for all \(t \in \bN\).
\end{theorem}
\begin{proof}
    Let \( \varphi:M(\cF) \to M(\cG)\) be a isomorphism of matroids.
    Then \( B_t^{\cG}= \bigcup_{\substack{J \in M(\cG)} \\ |J| \leq t} \Span(J) = \bigcup_{\substack{J \in M(\cG)}} \Span(\varphi(I)\). For all \( t \in \bN\) let \(M_t(\cF) \coloneqq \{I \in M(\cF) \mid |I| \leq t\}\). For the inclusion exclusion principle we have:
    \begin{align}
        |B^{\cF}_t| &= \sum_{\cX \subset M_t(\cF)} (-1)^{|\cX|+1}|\cap_{I \in \cX}\Span(I)| \\
        |B^{\cG}_t| &= \sum_{\cX \subset M_t(\cF)} (-1)^{|\cX|+1}|\cap_{I \in \cX}\Span(\varphi(I)|
    \end{align}
    Thus it is sufficient to prove that for every \(X \in M_t(\cF)\) we have 
    \(
    |\cap_{I \in \cX}\Span(I)|=|\cap_{I \in \cX}\Span(\varphi)|
    \)
    Which is only true if and only if \(\dim(\cap_{I \in \cX}\Span(I) = \dim(\cap_{I \in \cX}\Span(\varphi(I))\). Since \( \varphi^{-1}\) is also a matroid isomorphism we only need to show on of the two inequalities. \(\cap_{I \in \cX} \langle I \rangle = \{0\}\) If and only if it does not exists
\end{proof}



}


\newpage




\subsection*{possible defs}
{
\color{gray}

Since both the dimension of a linear code, and it's minimum Hamming distance are invariant by Hamming equivalence we can define:
\begin{definition}
    Let $\C$ be a linear code and $\bar \C$ its Hamming equivalence class then we define $\dim(\bar C) := \dim (C)$ and $d_H(\bar C) := d_H(\C)$.
   
\end{definition}

}




\subsection{r-weights}
\gr[]{Not sure where to put it, but I would probably remove the definition since we didn't use the concept that much}
{
\color{gray}
Given two spanning families, $\cF_1,\,\cF_2 \subset \Gr_1(V)$, it can sometimes be challenging to ascertain whether the projective metric \(w_{\cF_1}\) and \(w_{\cF_2}\) are equivalent . It proves useful to identify invariant properties of projective metrics through the equivalence relation.

\begin{definition}
    Given $f \in \cF$, we define the \myfont{r-weight} of $f$ as the projective weight of $f$ respect to the spanning family \(\cF\setminus\{f\}\) that is  $rw_{\cF}(f) := w_{\cF \setminus \{f\}}(f)$ if \(\Span(\cF\setminus \{f\}) = V\) and $rw_{\cF}(f) = +\infty$ otherwise.
\end{definition}

It can be easily seen that:
\begin{observation}
    If \(L:V \to V\) is an equivalence between $\cF_1$ and $\cF_2$ then for all $f \in \cF$
    \[
    rw_{\cF_1}(f) = rw_{\cF_2}(L(f))
    \]
\end{observation}

When the size of a projective metric is equal to $N+1$, the maximum r-weight of $\cF$ uniquely characterizes the projective metric. However, for larger sizes, this characterization no longer holds. 
\begin{observation}
    If $|\cF_1|=|\cF_2|=N+1$ then $\max_{f \in \cF_1}rw_{\cF_1}(f)=\max_{f \in \cF_1}rw_{\cF_1}(f)$ if and only if $w_{\cF_1} \cong w_{\cF_2}$
\end{observation}

}


\newpage



\section*{Constructing new metrics from old}


{
\color{blue}

\begin{lemma}\label{lem:subset complement bound}
Let $G$ be finite group and let $S, \cC, \cA  \subseteq G$ be subsets with the following properties: $c_1^{-1} c_2 \notin S$ for all distinct $c_1, c_2 \in \cC$ and $a_1 a_2^{-1} \in S$ for all $a_1, a_2 \in \cA$. Then 
\[
\card{\cC} \leq \frac{\card{G}}{\card{\cA}}.
\]
\end{lemma}

\begin{proof}
Consider the map $f: \cC \times \cA \to G: (c,a) \mapsto ca$. This map is injective because if $c_1 a_1 = c_2 a_2$ for distinct $c_1,c_2 \in \cC$ and $a_1,a_2 \in \cA$, then $c_1^{-1} c_2 = a_1 a_2^{-1}$, a contradiction. Hence $\card{\cC}\card{\cA} \leq \card{G}$.
\end{proof}

\begin{corollary}[\textbf{Code-Anticode bound}, \textcolor{red}{\textbf{Reference!!}}]
Let $G$ be a finite abelian group (or e.g. a module or vector space) with a translation-invariant distance function $d: G \times G \to \mathbb{R}$. Let $t$ be a positive integer. If $\cC$ is a code of minimum distance $t$ and $\cA$ a $(t-1)$-anticode, then
\[
\card{\cC} \leq \frac{\card{G}}{\card{\cA}}.
\]
This follows directly from lemma \ref{lem:subset complement bound} by considering the set $S$ to be the ball $\{x \in G | d(x,0)\leq t-1\}$ of radius $t-1$.
\end{corollary}
}

% \section*{General properties of codes}


% Many definitions that do not depend on the specific metric of the vector space, such as a generator matrix, parity check matrix, dual code can be taken the same as in the Hamming metric.
% \hsc[inline]{How do I write this clearly?}
% \gr[inline]{Maybe we should first see which definitions "behave well" with the projective spaces before leaving them the same? Like if I remember correctly the "Hamming dual" doesn't have nice proprieties respect to the projective metrics (although also all the other definitions we tried to give where not than nice either) I love this comment thingy}

% \subsection{Definitions}
% \begin{definition}
% Let $V$ be a $N$-dimensional vector space over $\Ff_q$ endowed with the $\F$-metric. A non-empty subset  $\Gamma \subseteq V$ is called a \myfont{$\bm{q}$-ary  $\bm{\F}$-(metric) code} of \myfont{length} $N$. The code is called \myfont{linear} if it is a linear subspace of $V$. The \myfont{minimum $\bm{\F}$-distance} $d_\F(\Gamma)$ of $\Gamma$ is defined as
% \[
% d_\F(\Gamma) = \min\{\,d_\F(x,y) \;\,|\;\, x,y \in \Gamma,\;  x \neq y\,\} \in \Nn^+
% \]
% if $|\Gamma| \geq 2$, and as $d_\F(\Gamma) = ??$ if $|\Gamma| = 1$. 
% \end{definition}

% \begin{observation}
% Let $\Gamma < V$ be a linear code, $\varphi$ a parent function for $\cF$ and $\C = \ker(\varphi)$. Then 
% \begin{equation}
%     d_{\cF}(\Gamma) = \min_{x \in \varphi^{-1}(\Gamma) \setminus \C }w_H(x)
% \end{equation}
% \end{observation}


% \newpage

\subsection{Other bounds}



\begin{definition}
Weight distribution, balls, spheres
\end{definition}

Sphere sizes for phase rotation metric/coset weight distribution of repetition code:

\[
S_k = \frac{1}{q}  \sum_{j=1}^q\left(
\binom{q}{j}  \prod_{i=0}^{j-1} \binom{\max(0,n+1-i(n+1-k))}{n+1-k}  \cdot  \sum_{\substack{c_1 + \ldots + c_{q-j} \,=\, n+1-j(n+1-k)\\ 0 \leq c_i \leq n-k}} \binom{n+1-j(n+1-k)}{c_1,\, c_2,\, \ldots,\, c_{q-j}}
\right) 
\]

For $q=2$ this reduces to
\begin{align*}
S_k &=   \binom{n+1}{n+1-k} \left( \sum_{\substack{c_1 \,=\,k\\ 0 \leq c_1 \leq n-k}} 1 \right) + \frac{1}{2}\binom{n+1}{n+1-k}\binom{k}{n+1-k}\left(\sum_{\text{empty sum } = n+1-2(n+1-k)} 1\right)\\
&= \begin{cases}
    \binom{n+1}{k} & \text{ if } k \leq \frac{n}{2} \\
    \frac{1}{2}\binom{n+1}{k} & \text{ if } k = \frac{n+1}{2} \text{ and $n$ odd}\\
    0 & \text{ if } k \geq \frac{n}{2}+1 \\
\end{cases}
\end{align*}
Maybe recursive formula?  Or simple formula for small radius (dependent on min distance of hamming code)\\
\\
%if metrics equivalent, families must have same same cardinality, 
number of $\wt = 1$ vectors is $(q-1)|\F|$? 

}



\newpage


{\color{gray}
\section{Information Set Decoding}



Relate decoder of an $\cF$ to decoders of related spanning families in the lattice


\begin{definition}
Support for vector
\end{definition}

}
